Non-line-of-sight imaging in the presence of scattering media using phasor fields

Non-line-of-sight (NLOS) imaging aims to reconstruct partially or completely occluded scenes. Recent approaches have demonstrated high-quality reconstructions of complex scenes with arbitrary reflectance, occlusions, and significant multi-path effects. However, previous works focused on surface scattering only, which reduces the generality in more challenging scenarios such as scenes submerged in scattering media. In this work, we investigate current state-of-the-art NLOS imaging methods based on phasor fields to reconstruct scenes submerged in scattering media. We empirically analyze the capability of phasor fields in reconstructing complex synthetic scenes submerged in thick scattering media. We also apply the method to real scenes, showing that it performs similarly to recent diffuse optical tomography methods.

==> sections/abstract.tex <==
Non-line-of-sight (NLOS) imaging aims to reconstruct scenes that are partially or completely occluded. Recent approaches have demonstrated high-quality reconstructions in complex scenes with arbitrary reflectances, occlusions and significant multipath. However, previous works have focused on surface scattering only, which reduces its generality in more challenging scenarios such as scenes with dense scattering media. In this work, we investigate how current state-of-the-art NLOS imaging methods, based on phasor fields, perform at reconstructing occluded scenes in the presence of scattering media. 
We empirically analyze the performance of phasor fields under controlled scenarios, and demonstrate the first results of NLOS imaging of complex scenes with turbid media. 


==> sections/conclusions.tex <==
% -
% Conclusions and discussion
% -

% \paragraph{Conclusions}
In conclusion, to the best of our knowledge, we have presented the first work aiming to reconstruct non-line-of-sight scenes in the presence of scattering media. For that, we have leveraged phasor fields for transforming the NLOS problem into a virtual LOS one, in which media results into an additional occluder. Our empirical analysis demonstrates that it is feasible to reconstruct NLOS scenes in very challenging visibility conditions, under a wide range of media properties. Moreover, we have shown that by increasing the reconstruction wavelength we can partially remove the contribution of the medium, at the price of a resolution loss. 
%

Our work is however limited by the same problems as LOS systems; therefore, for very thick media off-the-shelf phasor fields would fail at reconstructing the hidden scene (or said otherwise, it would only reconstruct the contribution of the media). However, given the flexibility of phasor fields for virtually developing complex optical systems, a very promising avenue of work is to translate current LOS methods for vision through scattering media to the phasor field domain. 

%Note that this also occurs with visible light.





% -
% Disclosures
% -

\paragraph{Funding. } 
Left blank during review. 
%This project has been funded by the European Research Council (ERC) under the EU’s Horizon 2020 research and innovation programme (project CHAMELEON, grant No 682080) and DARPA (project REVEAL, HR0011-16-C-0025).

\paragraph{Disclosures. } 
The authors declare no conflicts of interest.

==> sections/introduction.tex <==
%Transient imaging has recently allowed researches to exploit temporal information about the propagation of light, leveraging the amount of information that it is possible to extract and opening many new exciting applications (see~\cite{Jarabo_2017_STAR_Transient} for an in-depth review) including light-in-flight imaging~\cite{Velten2013femto, gkioulekas2015micron, gariepy2015single}, range sensing~\cite{bamji20140, kadambi2015frequency}, non-line-of-sight (NLOS) imaging~\cite{liu2019non, liu2020phasor, lindell2019wave, xin2019theory, o2018confocal, velten2012recovering, gupta2012reconstruction, laurenzis2014nonline, buttafava2015non} or material estimation~\cite{tsai2016shape, naik2014estimating}.
%To get access to this new information, some of the most representative transient imaging setups include streak-cameras~\cite{Velten2013femto}, laser gated systems~\cite{busck2004gated}, avalanche photodetectors~\cite{charbon2007will} (specifically single photon avalanche diodes (SPAD)~\cite{kirmani2014first, gariepy2015single}) or amplitude modulated continuous-wave (AMCW) systems~\cite{heide2013low, lin2014fourier}.

Recent advances on transient imaging~\cite{Jarabo_2017_STAR_Transient} using ultrafast sensors %such as streak cameras, gated sensors, or single-photon avalanche diodes 
have opened a wide range of novel imaging modalities, including the ability of imaging fully or partially occluded objects, or \emph{non-line-of-sight (NLOS) imaging}~\cite{velten2012recovering,gupta2012reconstruction, laurenzis2014nonline, buttafava2015non,o2018confocal,liu2019non,lindell2019wave,xin2019theory,heide2019non,liu2020phasor,iseringhausen2020non}, which has a large body of applications in medical imaging, autonomous driving, or surveillance and security, among others. 

Non-line-of-sight imaging aims for recovering occluded objects by using the light scattered from a secondary surface~\cite{maeda2019recent}. Most previous NLOS imaging approaches based on time-resolved information base on filtered backprojection using heuristic filters~\cite{velten2012recovering,laurenzis2014nonline,Arellano2017NLOS} or inverting ad-hoc light transport models~\cite{o2018confocal,xin2019theory,heide2019non,iseringhausen2020non}. Unfortunately, these approaches make assumptions on the scene being reconstructed, and present problems on hidden scenes with significant multiple scattering, anisotropic reflectance, occlusions and clutter. 
%
Recent wave-based models for NLOS imaging~\cite{liu2019non, lindell2019wave, liu2020phasor} have removed some of these limitations, by posing NLOS imaging as a \emph{virtual} wave propagation problem, effectively transforming NLOS imaging into a \emph{virtual} line-of-sight (LOS) problem. These algorithms have allowed NLOS imaging of real-world complex scenes at meter scale. 

Unfortunately, all these techniques so far assume lights travel on empty space, without the presence of any scattering media. This limits its applicability on real-world scenarios where turbid media might be significant, including driving through fog or medical imaging. However, seeing through turbid media is a challenge even in LOS setups, where many techniques have been proposed using optical coherence tomography (OCT)~\cite{huang1991optical,den1993location,han2000time,gibson2005recent,lindell2020three}, sparse coding in combination with time-of-flight cameras~\cite{heide2014imaging}, structured light~\cite{narasimhan2005structured}, coherent light modulation using spatial light modulators~\cite{vellekoop2007focusing}, or polarization~\cite{demos1997optical,schechner2001instant,treibitz2008active,Wu2018adaptive}. To the best of our knowledge, there is no existing work trying to see through media on NLOS configurations. 

In this letter we introduce the first analysis on NLOS imaging in the presence of scattering media. Given the amount of incoherent light due to scattering, we cannot rely on traditional inversion methods for NLOS imaging. Instead, we leverage recent advances on wave-based NLOS imaging, and in particular on the \emph{phasor field} formalism proposed by Liu et al.~\cite{liu2019non}: This framework allows us to create a virtual sensor on the visible surfaces, resulting on robust reconstruction of incoherent multiply scattered light. We demonstrate, for the first time, reconstructions of NLOS scenes in the presence of participating media of increasing density. We hope this will bridge the gap between  NLOS imaging and vision through scattering media, and foster new avenues of work in this field. 

%Among its applications, one that has had the most promising results when introducing temporal information is non-line-of-sight imaging, which analyze light scattered from multiples surfaces with the objective of recovering the geometry and visual appearance of objects outside the field of view of the sensor. While the use of this technology is fundamental in medical imaging, autonomous driving and many other domains, it remains a difficult challenge due to fact that inversion of light transport is an ill-posed problem.
%
%In the seminal work of Velten \etal~\cite{velten2012recovering} the authors proposed to use backprojection to reconstruct for the first time an isolated mannequin occluded from the sensor. Later on, their technique was accelerated by using GPU~\cite{Arellano2017NLOS}, made more efficient by using confocal measures~\cite{o2018confocal} and being able to recover the surfaces of hidden objects~\cite{xin2019theory,Young:2020:dlct}.
%The limitations of previous techniques were removed when the wave-based models were presented~\cite{liu2019non, lindell2019wave, liu2020phasor}, pushing the limit of the reconstructions to scenes at meters scale with a complexity never seen before. 

%While NLOS field is closely related to direct ranging and imaging through scattering media, the only sources of scattering in NLOS come from the hidden geometry and a diffuse thin visible plane.  In contrast when light travels inside media, it is scattered multiple times along its volume.
%
%The challenge of seeing in its presence can be even harder and several line-of-sight (LOS) approaches exists for solving it: an example of such techniques is Optical Coherence Tomography~\cite{huang1991optical}, which removes the light that arrives later than a specific time threshold, understanding that has been scattered inside the media and allowing to see in tissue with a great depth~\cite{han2000time} if there are enough ballistic photons. 
%In other scenarios dominated by diffusion, the halo generated by light can be used to track objects inside media~\cite{den1993location} or enhance the maximum depth in diffuse optical tomography techniques~\cite{gibson2005recent}.
%By using transient imaging, time-of-flight (TOF) cameras has allowed to see through a great depth in tissue using a sparse encoding~\cite{heide2014imaging}, using femto-photography to recover the rigid pose of a known geometry~\cite{raviv2014pose}, looking through a relative dense medium of 1.5 cm~\cite{satat2015imaging}, exploiting the fact of the different polarization of light in the transient regime to recover depth~\cite{Wu2018adaptive}, and using confocal diffuse tomography to see through a thick diffuser~\cite{lindell2020three}.

%While the above techniques have only been applied in line-of-sight scenarios, in this letter we propose to go one step further introducing the first analysis of looking through scattering media in non-line-of-sight imaging. An example of the setup of our experiments can be found in Fig. \ref{fig:teaser_setup}.
%Due to there isn't free space but participating media, NLOS methods that make assumptions about the number of scattering event cannot be used. For that reason, we rely on Phasor Fields~\cite{liu2019non} which is agnostic to the number of light bounces, by positioning a virtual sensor inside the scene, and also has been proven to be robust to incoherent scattering of light.
%We demonstrate that their theory can be applied in scenarios filled with participating media, achieving reconstructions of high quality, and that its application produces effects predicted by wave-propagation theory.






==> sections/introduction_copy.tex <==
Transient imaging has recently allowed researches to exploit temporal information about the propagation of light, leveraging the amount of information that it is possible to extract and opening many new exciting applications (see~\cite{Jarabo_2017_STAR_Transient} for an in-depth review) including light-in-flight imaging~\cite{Velten2013femto, gkioulekas2015micron, laurenzis2014nonline, gariepy2015single}, range sensing~\cite{bamji20140, kadambi2015frequency}, non-line-of-sight (NLOS) imaging~\cite{liu2019non, lindell2019wave, xin2019theory, o2018confocal, velten2012recovering, gupta2012reconstruction, laurenzis2014nonline, buttafava2015non} or material estimation~\cite{tsai2016shape, naik2014estimating}.
To get access to this new information, some of the most representative transient imaging setups include streak-cameras~\cite{Velten2013femto}, laser gated systems~\cite{busck2004gated}, avalanche photodetectors~\cite{charbon2007will} (specifically single photon avalanche diodes (SPAD)~\cite{kirmani2014first, gariepy2015single}) or amplitude modulated continuous-wave (AMCW) systems~\cite{heide2013low, lin2014fourier}.

% \adrian{This sentence makes little sense if in the previous paragraph we talked about "vision through turbid media". }
% When you applied these setups in presence of media, it tends to fail because of the number of scattering events that suffer the light in the volume of the media. As light travels through it, depending of the turbidity, it scatters producing a loss of coherence in the signal and because of that, a loss of visibility. To solve the challenge of visibility, one solution is taking into account the time of propagation of the light and remove the contribution of light scattered. 
Scattering media imposes new challenges because of the number of scattering events that happens in its transport inside of the volume. As light travels through it, depending of the turbidity, it scatters producing a loss of coherence in the signal resulting in a loss of visibility. 
While several approaches exists for solving the challenge, one solution adopted is taking into account the time of propagation of the light and remove the contribution of light scattered.
%
An example of such techniques is Optical Coherence Tomography~\cite{huang1991optical}, which removes the light that arrives later than a specific time threshold, understanding that has been scattered inside the media and allowing to see in tissue with a great depth~\cite{han2000time}.
% vision through turbid media~\cite{Wu2018adaptive, han2000time, heide2014imaging, raviv2014pose, satat2015imaging}
On the other side, the diffuse halo generated by light can be used to track objects inside media~\cite{den1993location} or enhance the maximum depth in diffuse optical tomography techniques~\cite{gibson2005recent}.
In the field of transient imaging, the use of time-of-flight (TOF) cameras has allowed to see through a great depth in tissue using a sparse encoding~\cite{heide2014imaging}, using femto-photography to recover the rigid pose of a known geometry~\cite{raviv2014pose}, looking through a relative dense medium of 1.5cm~\cite{satat2015imaging}, exploiting the fact of the different polarization of light in the transient regime~\cite{Wu2018adaptive}, and using confocal diffuse tomography to see through a thick diffuser~\cite{lindell2020three}.

%The main challenge of these methods is disambiguate the light that has been scattered from the direct coming from a surface. This challenge also exists in the field of reconstructing hidden geometry from the field of view of the camera (NLOS) and it is called Multi-Path Interference (MPI). 
Similar to the previous methods, non-line-of-sight field deals with reconstructing hidden geometry from the field of view of the camera by using the information of light that has been scattered in a thin diffuser. Even with the lost of coherency, NLOS methods have demonstrated their versality.
%
NLOS field started with the seminal work of Velten \etal~\cite{velten2012recovering}, where the authors proposed to use backprojection to recover shape from the arriving time of light coming to a transient sensor. %This method was later extended to use not only streak-cameras but also gated-systems~\cite{laurenzis2014nonline}, SPADs~\cite{buttafava2015non} and later to be more efficient using GPU~\cite{Arellano2017NLOS}.\adrian{Missing Gordon's papers (CNLOS, f-k migration) and Fermat Paths; also I think the pitch shouldn't be the sensor they use, but the technique}
%
This starting approach was later improved by making it faster on GPU~\cite{Arellano2017NLOS}, by using confocal measures~\cite{o2018confocal}, by reconstructing the surfaces of the hidden objects~\cite{xin2019theory}, and by using a wave-based image formation model~\cite{liu2019non,lindell2019wave}.

The latest advances in the NLOS field have made it possible to reconstruct robustly geometry at meters scale and with the presence of strong interreflexions (MPI). Although the complexity of the scenes is higher than ever, all the scenarios analyzed consist on light moving on free space between the different surfaces. In fact, they assume as sources of scattering only the diffuser and the geometry. 
%
In this letter we present the first analysis of NLOS reconstructions in the presence of scattering media by adding a layer of complexity caused by the new source of scattering and showing how it is possible to imaging even in that situations.
To do that, we rely on Phasor Fields technique~\cite{liu2019non} which moves the NLOS challenge to the line-of-sight (LOS) field by positioning a virtual sensor, and hence being agnostic to the number of scattering events of the light. Additionally its robustness to MPI made it ideal when dealing with scattering media.

%
%NLOS methods based in the seminal work of Velten \etal~\cite{velten2012recovering}, that uses backprojection to recover shape from the arriving time of the light to the transient sensor. This method was later extended to use not only streak-cameras but also gated-systems \cite{laurenzis2014nonline} and SPADs \cite{buttafava2015non} and later to be more efficient using GPU \cite{Arellano2017NLOS}.
%
% Until recently, NLOS methods only could work in lab conditions (without the presence of strong MPI) based in the seminal work of Velten \etal~\cite{velten2012recovering}, that uses backprojection to recover shape from the arriving time of the light to the transient sensor. This method was later extended to use not only streak-cameras but also gated-systems \cite{laurenzis2014nonline} and SPADs \cite{buttafava2015non} and later to be more efficient using GPU \cite{Arellano2017NLOS}.
%
% \adrian{Now we talk about NLOS? But our goal wasn't turbid media? I'm more and more convinced that our pitch should be NLOS (or imaging through diffusers) in turbid media} Until recently, NLOS methods only could work in lab conditions (without the presence of strong MPI). This limitation of previous work was removed in the work of Liu \etal~\cite{liu2019non} where the authors presented Phasor Fields, a novel technique that moves the challenge to the line-of-sight (LOS) imaging field allowing to be agnostic about the number of scattering events of the light or the presence of occluders.

% In this letter we propose to understand the problem of looking through a turbid medium from another perspective, translating the challenge towards looking through an occluder. To do that, we rely on the work of Liu \etal~\cite{liu2019non}, which has been proved to work in complex scenarios without the presence of media and being able to deal with MPI. The combination of both properties made it ideal in the scenario of strong scattering.\adrian{Rewrite when pitch is final!}

% In this letter we propose to understand the problem of looking through a turbid media from another perspective, translating the challenge towards looking through an occluder. To do that, we rely on the work of Liu \etal~\cite{liu2019non}, extending it to scenarios with the presence of turbid media and analyzing the reconstructions achieved. Also, we propose a posteriori filtering that enhance reconstruction visualization. 
% This work is a first step in the development of robust media imaging techniques using transient imaging.

==> sections/method.tex <==
\paragraph{Experimental design. } 
We use two different types of scenes (see Figure~\ref{fig:geometry_scenes}): The simplest one contains only a planar Z-letter in front of the diffuser at a distance of 2 meters, while the complex one contains a room with a shelf at the back wall, at 1.8 meters from the diffuser. The \textit{Z scene} allows us to study how the medium affects visibility in the phasor fields domain. On the other hand, the \textit{shelf scene} features occlusions and multipath illumination, resulting into a more challenging scenario, and serves us to validate the concussions found in the Z scene in more complex setups. 
%
Controlling the properties of scattering media is hard in practice; therefore we opt for using carefully controlled data from simulation. We use a publicly available transient renderer~\cite{Jarabo2014transient} to compute the impulse response $H(x_p \rightarrow x_c, t)$ of the hidden scenes. We compute each impulse response for $128^2$ laser positions $x_p$ equally spaced in a grid along the relay wall, and captured in a single SPAD point $x_c$. The temporal resolution is 4096 bins, each with a temporal resolution of about 3ms. 

We characterize the media by using their bulk optical parameters following the radiative transfer framework. In particular, we use the extinction coefficient $\sigma_t = \sigma_a + \sigma_s$ and scattering albedo $\alpha = \sigma_s / \sigma_t$, with $\sigma_a$ and $\sigma_s$ the absorption and scattering coefficients, respectively. 
%
As the media's phase function, we use the empirical model proposed by Henyey and Greenstein~\cite{henyey1941diffuse}, which allows to model anisotropic scattering using the anisotropy factor $g\in(-1,1)$, where $g>0$, $g=0$ and $g<0$ model forward, isotropic and backward scattering respectively. Unless stated otherwise we assume an isotropic phase function. In all cases we assume homogeneous media. 

\begin{figure}[t]
\centering
\includegraphics[width=.3\columnwidth]{figures/pf_m1_atFront}
\includegraphics[width=.3\columnwidth]{figures/shelves/pf_m4_atFront.png}
    \caption{Baseline non-line-of-sight reconstructions using phasor fields of the \emph{Z scene} (left) and the \emph{shelf scene} (right) without scattering media.}
    \label{fig:nomedia}
\end{figure}
%
\paragraph{Reconstruction. } 
We reconstruct a voxelization of the scene by sequentially focusing the virtual imaging system on each reconstructed voxel. The voxel resolution is $73\times59\times73$ for the \emph{Z scene} and $142\times142\times142$ for the \emph{shelf scene}. We use a Matlab implementation of phasor fields with the solver based on backprojection, though more efficient solvers could be used for faster performance~\cite{liu2020phasor}. The reconstruction costs depends on the total resolution of the scene: On an Intel Xeon E5 with 256GB RAM the \emph{Z scene} takes 29s and the \emph{shelf scene} takes 254s. Figure~\ref{fig:nomedia} shows baseline reconstructions of both scenes without media.

We set the reconstruction wavelength $\lambda$ according to the resolution following Liu et al.~\cite{liu2019non}, to $\lambda = 4 \, \Delta_c$ with $\Delta_c$ the resolution of the sample points on the relay wall. Similar to traditional LOS Fourier optics, the wavelength defines the maximum resolution of the reconstruction. As we show later, choosing a larger phasor field wavelength allows for removing part of the media contribution, at the cost of reducing the resolution of the reconstruction. 

For visualization, we remove the contribution of the extinction of med medium by filtering the final reconstruction as a post-process. We exploit the spatial information of the voxels, as well as the properties of the medium, and apply the following scale factor $K(x_v)$ per-voxel:
\begin{equation}
  K(x_v) = \frac{1 - (\alpha \, e^{- d(x_v)\,\alpha })}{e^{-d(x_v)\,\sigma_t}} ,
\end{equation}
which depends on the distance $d(x_v)$ from the center of the relay wall (the diffuser) to the voxel $x_v$. This factor depends on the properties of the medium: If they were unknown, they should be estimated from the reconstruction. 
%Figure \ref{fig:setup_orientations_visualization} show the different views of the scenes we will using in the analysis. Additionally, Figure \ref{fig:teaser_filtering} shows a comparison between the raw and filtered reconstruction. 

% We apply both kernels calculating the distance $d$ from the center of the diffuser to the center of each voxel. Notice that these kernels doesn't help in the presence of multiple scattering and it is necessary to know the coefficients of the medium (or approximate them).


==> sections/overview.tex <==
% -
% Overview
% -


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/setup_productionX.png}
    \caption{\textbf{Problem setup} We aim to image a scene hidden behind a diffuser, with the hidden scene filled with scattering medium. For that, we image the diffuser with a laser emitter and an ultrafast imaging device located outside of the medium. }
    \label{fig:teaser_setup}
\end{figure}

Non-line-of-sight imaging using \emph{phasor fields}~\cite{liu2019non} is based on the observation that, by convolving a time-resolved optical carrier with a monochromatic phasor, we can model the propagation of this virtual phasor using a Rayleigh-Sommerfeld Diffraction (RSD)-like operator to propagate this virtual wave. The immediate consequence is that we can use well-known tools from Fourier optics for modeling the phasor propagation. 
%
Therefore, if we measure the linear light transport matrix~\cite{ng2003all} in the occluder, we can pose the NLOS imaging problem as a \emph{virtual} line-of-sight setup. 

Let us define the phasor $\mathcal{P}_{\omega}(x, t)$ at point $x$ and time $t$, and with frequency $\omega$ as
%
\begin{equation}
  \mathcal{P}_{\omega}(x, t) \equiv \mathcal{P}_{0, \omega} (x) \, e^{i \omega t} ,
\end{equation}
%
with $\mathcal{P}_{0, \omega} (x)$ and $e^{i \omega t}$ the intensity and phase at the instant $t$ of the phasor, we can model the propagation from a surface $S$ to a point $x_d\in D$ of this virtual wave field $\mathcal{P}_{\omega}(x, t)$  as
\begin{equation}
  \mathcal{P}_\omega({x}_d,t) =\gamma \int_{S} {\mathcal{P}_\omega({x}_s,t)\frac{e^{ik|{x}_d-{x}_s|}}{|{x}_d-{x}_s|} \, d{x}_s}.
\label{eq:rsd}
\end{equation}
%
where $\gamma\approx 1 / \mid \left< S \right> - x_d \mid$ is an attenuation factor, $k = 2\pi / \lambda$ is the wavelength number with $\lambda=2\pi / \omega$, $x_s \in S$ and $x_d \in D$. Equation~\eqref{eq:rsd} is similar to the RSD operator. For generality, in the following we remove the frequency dependence from the phasor, to account for non-monochromatic phasors. 

In order to image a hidden scene from a virtual camera with aperture placed at surface $C$, we first need to compute the incoming phasor field on the virtual sensor $\mathcal{P}(x_c, t)$ with $x_c \in C$ as a function of a phasor $\mathcal{P}(x_p, t)$ in the virtual emitter on surface $P$. This is computed by leveraging the linearity and time-invariance of light transport, using the impulse response of the hidden scene $H(x_p \rightarrow x_c, t)$ to compute $\mathcal{P}(x_c, t)$ as
\begin{equation}
    \mathcal{P}(x_c,t) =
    \int_P \left[\mathcal{P}(x_p,t) \star H(x_p \rightarrow x_c, t)\right] \, dx_p ,
\end{equation}
where $\star$ denotes the convolution operator. Finally, to generate the image of the hidden scene $I(x_v)$ as seen from the virtual sensor, with $x_v$ the point being reconstructed, an image formation model $\Phi(\cdot)$ is applied over $\mathcal{P}\left(x_c, t\right)$ as:
\begin{equation}
  I(x_v) = \Phi\left(\mathcal{P}\left(x_c, t\right)\right) .
\end{equation}
The image formation function $\Phi(\cdot)$ depends on the type of imaging system implemented (details in~\cite{liu2019non}). In our work we use a virtual confocal time-gated camera, by setting the emitter phasor $\mathcal{P}(x_p, t)$ and image formation function $\Phi(\mathcal{P}(x_c, t))$ to: 
%
\begin{equation}
  \mathcal{P}(x_p, t) = e^{i \omega (t - \frac{1}{c} \mid x_v - x_p \mid)} e^{- \frac{(t - t_0 - \frac{1}{c} \mid x_v - x_p \mid)^{2}}{2 \sigma^{2}}} ,
    \label{eq:phasor_emision}
\end{equation}
\begin{equation}
    \Phi(\mathcal{P}(x_c, t)) = \left| \; \; \mathcal{R}_{x_v}(\mathcal{P}(x_c, -\frac{1}{c} \mid x_v - x_c \mid)) \; \; \right|^{2} ,
    \label{eq:imageFormationModel}  
\end{equation}
%
where $c$ is the light speed in vacuum and $\mathcal{R}_{x_v}$ is the RSD operator

% -
% Explanation of test scenes
% - 

While phasor fields have been demonstrated very effective at reconstructing NLOS scenes in empty space, no work has been done scenes filled with scattering media, which results in more challenging visibility conditions. Here we analyze the performance of phasor fields on that context, by imaging a scene filled with scattering media of increasing density hidden behind a diffuser (which acts as \emph{relay wall}). This diffuser will serve as our virtual illumination and camera on the phasor field domain. A setup of the scene is shown in Figure \ref{fig:teaser_setup}. In the following, we describe in depth our setup and experiments, and analyze the results of the reconstructions. 


\begin{figure}
  \centering
  \captionsetup[subfigure]{justification=centering}
  % \begin{subfigure}{.5\columnwidth}
  %   \centering
  %   % include second image
  %   \includegraphics[width=.95\linewidth]{figures/setup_z.png}  
  %   % \caption{Simple scene}
  %   \label{fig:sub-second}
  % \end{subfigure}%
  % \begin{subfigure}{.5\columnwidth}
  %   \centering
  %   % include second image
  %   \includegraphics[width=.95\linewidth]{figures/setup_shelves.png}  
  %   % \caption{Complex scene}
  %   \label{fig:sub-second}
  % \end{subfigure}
  \includegraphics[width=\columnwidth]{figures/setup_figure.pdf}
  \caption{We use two scenes in our experiments: (Left) a simple scene consisting of a single planar letter behind the diffuser (in green), and (right) a more complex scene of a closed room (walls in grey) with a shelf (red) on the back wall. }
  \label{fig:geometry_scenes}
\end{figure}

==> sections/results.tex <==



\begin{figure}[t]
    \setlength{\tabcolsep}{2pt}
    \graphicspath{{figures/}}
    \centering
    \begin{tabular}{cccccc}
       & $\alpha=0.15$ & 0.33 & 0.5 & 0.67 & 0.83 \\
      \rotatebox[origin=c]{90}{$\sigma_t=0.5$} & \tableFig{density/0.5/pf_m1_filtered_atFront.png}{5em} & \tableFig{density/0.5/pf_m2_filtered_atFront.png}{5em} & \tableFig{density/0.5/pf_m3_filtered_atFront.png}{5em} & \tableFig{density/0.5/pf_m4_filtered_atFront.png}{5em} & \tableFig{density/0.5/pf_m4_filtered_atFront.png}{5em} \\
      \rotatebox[origin=c]{90}{$\sigma_t=1.0$} & \tableFig{density/1/pf_m1_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m2_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m3_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m4_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m5_filtered_atFront.png}{5em} \\
      \rotatebox[origin=c]{90}{$\sigma_t=2.0$} & \tableFig{density/2/pf_m1_filtered_atFront.png}{5em} & \tableFig{density/2/pf_m2_filtered_atFront.png}{5em} & \tableFig{density/2/pf_m3_filtered_atFront.png}{5em} & \tableFig{density/2/pf_m4_filtered_atFront.png}{5em} & \tableFig{density/2/pf_m5_filtered_atFront.png}{5em} \\
      % \rotatebox[origin=c]{90}{4.0} & \tableFig{density/4/pf_m1_filtered_atFront.png}{5em} & \tableFig{density/4/pf_m2_filtered_atFront.png}{5em} & \tableFig{density/4/pf_m3_filtered_atFront.png}{5em} & \tableFig{density/4/pf_m4_filtered_atFront.png}{5em} & \tableFig{density/4/pf_m5_filtered_atFront.png}{5em} \\
    \end{tabular}
    \caption{Non-line-of-sight reconstructions using phasor fields of the \emph{Z scene} in the presence of scattering media, for varying extinction $\sigma_t$ (rows, in m$^{-1}$) and scattering albedo $\alpha$ (columns, unitless). As the medium gets more scattering (increasing albedo), the coherence of the signal degrades; this is specially noticeable with denser media (higher $\sigma_t$), where the number of scattering events is larger. This behavior is similar to the effect of scattering media in line-of-sight modalities. }
    \label{fig:density_results}
  \end{figure}

  \paragraph{Analysis.} 
Figure~\ref{fig:density_results} shows the results of phasor fields when reconstructing the simple \emph{Z scene} as a function of different media densities (its extinction coefficient $\sigma_t$) and relative amount of scattering (its scattering albedo $\alpha$). For low scattering albedo, as the media thickness (its extinction coefficient, which is directly related with media density) increases the signal's amplitude is attenuated, though the coherence remains, so it is still possible to reconstruct a sharp image. In contrast, higher scattering albedos result into less coherence, resulting into a frequency loss. 

% Moreover, when in Phasor Fields the virtual complex field is propagated, it is done by using wave theory accounting for the interferences in the field. This produces two effects: on one hand, speckles appear from the interference given the coherent (laser) illumination. These speckles will appear as the medium becomes more turbid, and their appearance indicates that even in a highly turbid medium, signal's phase coherence is preserved.
  %In addition, with an increase in the turbidity of the medium, speckles begin to appear as coherent noise. These speckles have statistical properties and could be used to improve the recovery of the signal hidden in them.
%  On the other hand, the phenomenon of coherent backscattering will also appear. This effect is characterized by signal interference, which generates an increase of the energy in the direction of return in its trajectory. This effect can be seen in the reconstructions as an increase of the light energy next to the diffuser and is dependent on how much energy is dispersed backwards and the number of interactions the light has in its path.


Figure~\ref{fig:anisotropy_results} shows the effect on the reconstructions of the phase function's anisotropy. For forward scattering, the energy penetrates deeper into the medium, while backward scattering results into more scattering near the virtual camera, and therefore poorer visibility conditions. This shows that similarity theory~\cite{wyman1989similarity}, which is well-known from traditional optics, does also hold on the phasor fields realm. 


%  Although no such structure appears in the reconstructions, anisotropy still influences the quality of reconstructions: if the media have a dominant forward scattering, more energy will penetrate the medium without being reflected and the reconstruction quality improves. On the other hand, with dominant back scattering more energy will come back to the sensor resulting in more media being reconstructed and consequently hiding the geometry.

  \begin{figure}[t]
    \setlength{\tabcolsep}{2pt}
    \graphicspath{{figures/}}
    \centering
    \begin{tabular}{cccccc}
       & $\alpha=0.15$ & 0.33 & 0.5 & 0.67 & 0.83 \\
       \rotatebox[origin=c]{90}{$g = 0.7$} & \tableFig{forwardScattering/pf_m1_filtered_atFront.png}{5em} & \tableFig{forwardScattering/pf_m2_filtered_atFront.png}{5em} & \tableFig{forwardScattering/pf_m3_filtered_atFront.png}{5em} & \tableFig{forwardScattering/pf_m4_filtered_atFront.png}{5em} & \tableFig{forwardScattering/pf_m5_filtered_atFront.png}{5em} \\
       \rotatebox[origin=c]{90}{$g = 0$} & \tableFig{density/1/pf_m1_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m2_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m3_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m4_filtered_atFront.png}{5em} & \tableFig{density/1/pf_m5_filtered_atFront.png}{5em} \\
       \rotatebox[origin=c]{90}{$g = -0.7$} & \tableFig{backscattering/pf_m1_filtered_atFront.png}{5em} & \tableFig{backscattering/pf_m2_filtered_atFront.png}{5em} & \tableFig{backscattering/pf_m3_filtered_atFront.png}{5em} & \tableFig{backscattering/pf_m4_filtered_atFront.png}{5em} & \tableFig{backscattering/pf_m5_filtered_atFront.png}{5em} \\
    \end{tabular}
    \caption{Non-line-of-sight reconstructions using phasor fields of the \emph{Z scene} in the presence of scattering media, for fixed extinction $\sigma_t=1$ m$^{-1}$, and varying scattering albedo $\alpha$ (columns, unitless) and phase function's anisotropy $g$ (rows, unitless). The media range from forward scattering ($g=0.7$) to backward scattering ($g=-0.7$); isotropic scattering is $g=0$. As expected from similarity theory~\cite{wyman1989similarity}, the net effect of the phase function is a larger penetration for forward scattering (top), and an effectively thicker medium for backward scattering. }
    \label{fig:anisotropy_results}
  \end{figure}


Now we analyze the effect of the wavelength $\lambda$ on the reconstruction, and in particular how increasing its value allows for deeper penetration on the medium. Figure~\ref{fig:wavelength_results} compares the reconstruction in a very scattering medium ($\sigma_t=1 $ m$^{-1}$, $\alpha=0.87$) for increasing $\lambda$. In particular, we double and triple the optimal wavelength defined by $\lambda=4\,\Delta_c$: While this results into a resolution loss, visible as smoother reconstructions, we can observe that by increasing the wavelength we can recover geometry more clearly geometry hidden by the scattering in the medium. 
%
  \begin{figure}[t]
    \setlength{\tabcolsep}{2pt}
    \graphicspath{{figures/}}
    \centering
    \begin{tabular}{ccc}
       $\lambda = \lambda_0$ & $\lambda = 2\,\lambda_0$ & $\lambda = 3\,\lambda_0$ \\
       \tableFig{density/1/pf_m5_filtered_atFront.png}{8em} & \tableFig{lambdax2/1/pf_m5_filtered_atFront.png}{8em} & \tableFig{lambdax4/1/pf_m5_filtered_atFront.png}{8em} \\ 
    \end{tabular}
    \caption{Reconstructions with phasor fields of the \emph{Z scene} in the presence of a scattering medium with extinction $\sigma_t = 1$ m$^{-1}$ and scattering albedo $\alpha = 0.83$ for increasing wavelength $\lambda$, with baseline $\lambda_0=4\,\Delta_c= 0.11$ m. Higher values of $\lambda$ result into deeper penetration through the medium, at the cost of lower spatial resolution on the reconstruction. }
    \label{fig:wavelength_results}
  \end{figure}

  
Finally, we analyze how our experiments extrapolate to scenes with significantly more complexity. Figure~\ref{fig:shelves_results} shows the non-line-of-sight reconstruction of a more complex scene, with significant surface-to-surface multipath, in addition to multiple scattering in the medium. This results in larger indirect contribution on the medium, thus resulting in more challenging visibility conditions. As our results show, even for relatively thick media we can reconstruct such complex scene with good quality. 

\newcommand{\sizeShelf}{.28\columnwidth}
  \begin{figure}[t]
    \setlength{\tabcolsep}{2pt}
    \graphicspath{{figures/}}
    \centering
    \begin{tabular}{cccc}
      %  & 0.15 & 0.33 & 0.5 & 0.67 & 0.83 \\
       \rotatebox[origin=c]{90}{No media} & \tableFig{shelves/pf_m4_atFront.png}{\sizeShelf} & \tableFig{shelves/pf_m4_atLateral.png}{\sizeShelf} & \tableFig{shelves/pf_m4_atOrto.png}{\sizeShelf} \\ 
       \rotatebox[origin=c]{90}{$\sigma_t = 1$} & \tableFig{shelves/pf_m1_filtered_atFront.png}{\sizeShelf} & \tableFig{shelves/pf_m1_filtered_atLateral.png}{\sizeShelf} & \tableFig{shelves/pf_m1_filtered_atOrto.png}{\sizeShelf} \\
       \rotatebox[origin=c]{90}{$\sigma_t = 1.5$} & \tableFig{shelves/pf_m2_filtered_atFront.png}{\sizeShelf} & \tableFig{shelves/pf_m2_filtered_atLateral.png}{\sizeShelf} & \tableFig{shelves/pf_m2_filtered_atOrto.png}{\sizeShelf}  \\
       
    \end{tabular}
    \caption{Non-line-of-sight reconstruction of the \emph{shelf scene} in the presence of media of increasing density: From top to bottom, $\sigma_t=0$ (no media), $\sigma_t=1$, and $\sigma_t=1.5$. In all cases, the scattering albedo is fixed to $\alpha=0.5$. Each column shows different views of the reconstruction (front, top, and perspective respectively). }
    \label{fig:shelves_results}
  \end{figure}
  
  
  
 
